ClueWeb22: 10 Billion Web Documents with Visual and Semantic Information

ClueWeb22, the newest iteration of the ClueWeb line of datasets, provides 10 billion web pages affiliated with rich information. Its design was influenced by the need for a high quality, large scale web corpus to support a range of academic and industry research, for example, in information systems, retrieval-augmented AI systems, and model pretraining. Compared with earlier ClueWeb corpora, the ClueWeb22 corpus is larger, more varied, of higher-quality, and aligned with the document distributions in commercial web search. Besides raw HTML, ClueWeb22 includes rich information about the web pages provided by industry-standard document understanding systems, including the visual representation of pages rendered by a web browser, parsed HTML structure information from a neural network parser, and pre-processed cleaned document text to lower the barrier to entry. Many of these signals have been widely used in industry but are available to the research community for the first time at this scale.

==> Sections/benchmark.tex <==
\section{Planned Benchmarking Tasks}


==> Sections/scenarios.tex <==
\section{Usage Scenarios and Benchmarks}
\label{sec:usage}

\cx{I think we should discuss the already done work here, instead of guessing what's going to happen?}

\cx{Or we mainly focus on referring to existing benchmarks and keep updating this paper or just the git repo will do?}







==> Tables/annotation_a.tex <==
\begin{table}[t]
    \centering
    \small
        \caption{Semantic Annotation Count Stats of ClueWeb22 SeA.}
    \label{tab:size}
    \begin{tabular}{lllll}
    \toprule
    \textbf{Annotation} & \textbf{Total} & \textbf{Avg. Per Document} & \textbf{Stdev.}  \\ \hline
        Title &  1.4B  & 0.8 & 0.6\\ 
        Heading &  19.8B  & 11.0 & 16.7\\ 
        Paragraph &  14.3B  & 7.9 & 17.6\\ 
        List &  1.7B  & 1.0 & 3.6\\ 
        Table &  1.4B  & 0.8 & 3.3\\ 
         \bottomrule
    \end{tabular}
\end{table}

==> Tables/annotation_l.tex <==
\begin{table}[t]
    \centering
    \small
        \caption{Semantic Annotation Count Stats of ClueWeb22 SeA.}
    \label{tab:size}
    \begin{tabular}{lllll}
    \toprule
    \textbf{Annotation} & \textbf{Total} & \textbf{Avg. Per Document} & \textbf{Stdev.}  \\ \hline
        Title &  6.6B  & 0.8 & 0.6\\ 
        Heading &  71.8B  & 9.0 & 14.8\\ 
        Paragraph &  104.5B  & 13.1 & 26.5\\ 
        List &  4.9B  & 0.6 & 2.8\\ 
        Table &  7.2B  & 0.9 & 4.1\\ 

         \bottomrule
    \end{tabular}
\end{table}
